Analytical Derivation and Comparison of Alarm Similarity Measures

An industrial process includes many devices, variables, and sub-processes that are physically or electronically interconnected. These interconnections imply some level of correlation between different process variables. Since most of the alarms in a process plant are defined on process variables, alarms are also correlated. However, this can be a nuisance to operators, for one fault might trigger a, sometimes large, number of alarms. So, it is essential to find and correct correlated alarms. In this paper, we study different methods and techniques proposed to measure correlation or similarity between alarms. The similarity indices are first analytically calculated and then studied and compared. The results are also validated using Monte-Carlo simulation.

==> biblio.tex <==
\begin{thebibliography}{99}
\bibitem{ci20}
Hollifield, B.R. and Habibi, E., \textit{Alarm Management: A Comprehensive Guide: Practical and Proven Methods to Optimize the Performance of Alarm Management Systems}, ISA, 2010.

\bibitem{izadi-intro} I. Izadi, S. L. Shah, D. S. Shook, and T. Chen, ``An introduction to alarm analysis and design," \textit{IFAC Proceedings}, vol.~42, no.~8, pp.~645--650, 2009.

\bibitem{Li}
Li, Tingshun, Wen Tan, and Xiaojie Li. ``Data mining algorithm for correlation analysis of industrial alarms,'' \textit{Cluster Computing}, pp.~1--11, 2017.

\bibitem{Yu}
Yu, Y., Zhu, D., Wang, J. and Zhao, Y., ``Abnormal data detection for multivariate alarm systems based on correlation directions,'' \textit{Journal of Loss Prevention in the Process Industries}, vol.~45, pp.~43--55, 2017.

\bibitem{ci7}
Yang, F., Shah, S.L., Xiao, D. and Chen, T., ``Improved correlation analysis and visualization of industrial alarm data,''  \textit{ISA Transactions}, vol.~51, pp.~499--506, 2012
\bibitem{ci5}
Noda, M., Higuchi, F., Takai, T. and Nishitani, H., ``Event correlation analysis for alarm system rationalization,''  \textit{Asia Pacific Journal of Chemical Engineering}, vol.~6, pp.~497--502, 2011

\bibitem{ISA18.2} International Society of Automation (ISA), \textit{Management of alarm systems for the process industries,} ANSI/ISA Standard 18.2, 2009.  

\bibitem{ci30}
Downs, J.J. and Vogel, E.F., ``A plant-wide industrial process control problem,''  \textit{Computers \& Chemical Engineering}, vol.~17, pp.~245--255, 1993.

\bibitem{ci6}
Nishiguchi, J. and Takai, T., ``IPL2 and 3 performance improvement method for process safety using event correlation analysis,''  \textit{Computers \& Chemical Engineering}, vol.~34, pp.~2007--2013, 2010.

\bibitem{ci11}
Su, J., Wang, D., Zhang, Y., Yang, F., Zhao, Y. and Pang, X., ``Capturing Causality for Fault Diagnosis Based on Multi-Valued Alarm Series Using Transfer Entropy,''  \textit{Entropy}, vol.~19, p.~663, 2017.

\bibitem{ci8}
Higuchi, F., Yamamoto, I., Takai, T., Noda, M. and Nishitani, H., ``Use of event correlation analysis to reduce number of alarms,'' \textit{Computer Aided Chemical Engineering}, vol.~27, pp.~1521--1526, 2009.

\bibitem{ci9}
Kondaveeti, S.R., Izadi, I., Shah, S.L. and Black, T., ``Graphical representation of industrial alarm data,''  \textit{IFAC Proceedings Volumes}, vol.~43, pp.~181--186, 2010.

\bibitem{Hu-delay} 
Hu, W., Wang, J. and Chen, T., ``A new method to detect and quantify correlated alarms with occurrence delays,'' \textit{Computers \& Chemical Engineering}, vol.~80, pp.189--198, 2015.

\bibitem{ahmed}
Ahmed, K., Izadi, I., Chen, T., Joe, D., Burton, T., ``Similarity Analysis of Industrial Alarm Flood Data,'' \textit{IEEE Transactions on Automation Science and Engineering}, vol.~10, pp.~452--457, 2013.

\bibitem{Yang}
Yang, Z., Wang, J. and Chen, T., ``Detection of correlated alarms based on similarity coefficients of binary data,'' \textit{IEEE Transactions on Automation science and Engineering}, vol.~10, pp.~1014--1025, 2013.

\bibitem{ci10}
Choi, S.S., Cha, S.H. and Tappert, C.C., ``A survey of binary similarity and distance measures,''  \textit{Journal of Systemics, Cybernetics and Informatics}, vol.~8, pp.~43--48, 2010.


\bibitem{ci4}
Yang, F., Shah, S.L. and Xiao, D., ``Correlation analysis of alarm data and alarm limit design for industrial processes,'' in \textit{Proceedings of the American Control Conference (ACC)}, pp.~5850--5855, 2010.


%\bibitem{ci3}
%Izadi, I., Shah, S.L., Shook, D.S., Kondaveeti, S.R. and Chen, T., ``A framework for optimal design of alarm systems,''  \textit{IFAC Proceedings Volumes}, 42(8), pp.651-656, 2009


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\bibitem{ci1}
%Goel, P., Datta, A. and Mannan, M.S., ``Industrial alarm systems: Challenges and \mbox{opportunities},''  \textit{Journal of Loss Prevention in the Process Industries}, 50, pp.23-36, 2017

%\bibitem{cip1}
%Stauffer, T. and Clarke, P., ``Using alarms as a layer of protection,''  \textit{Process Safety Progress}, 35(1), pp.76-83, 2016

%\bibitem{ci2}
%Izadi, I., Shah, S.L., Shook, D.S. and Chen, T., ``An introduction to alarm analysis and design,''  \textit{IFAC Proceedings Volumes}, 42(8), pp.645-650, 2009

%\bibitem{ci21}
%Gao, H., Xu, Y. and Zhu, Q., ``Spatial interpretive structural model identification and AHP-based multimodule fusion for alarm root-cause diagnosis in chemical processes,''  \textit{Industrial \& Engineering Chemistry Research}, 55(12), pp.3641-3658, 2016

\end{thebibliography}

